A Threat Modeling Framework for Evaluating Computing Platforms Against Architectural Attacks

software component misuse a privileged relationship with the hardware to by pass system protections, monitors, or forensic tools. These relationships are often not illegal and exist between system components by design. Hence, even a system with secure hardware and software components, can be architecturally vulnerable. Unfortunately, the existing threat modeling schemes are not applicable for modeling architectural attacks against computing platforms. This is mostly because the existing techniques rely on an abstract representation of a software (.e.g., Data Flow Diagram) as a primary requirement which is not available for a platform as a whole (considering both hardware and software elements). In this paper, we have discussed the necessity of a hardware-software architectural view to system threat modeling. Then, we have proposed Lamellae, a framework adapts threat modeling method to be applicable for untrusted platforms by a holistic approach. Lamellae involves system security architecture for abstract modeling of the platforms. Using the Design structure matrix analysis, Lamellae helps an end-user to identify possible attack vectors against a platform. The framework is a connection point of concepts from system engineering and software security domains. We have applied the framework on a multi-purpose computer with x86-64 architecture as a case-study to show the effectiveness of our framework.

==> boot.tex <==
\begin {figure}[ht]
\begin{center}
\smartdiagramset{uniform sequence color=true,
sequence item border color=black,sequence item font size=\tiny,
sequence item text color=white
}
\smartdiagram[sequence diagram]{Reset vector, CPU mode switch, cpu/chipset initialization, Memory initialization, Switch to RAM, Platform enabling, Int enabling, Timer initialization, Memory caching control initialization, AP initialization, Simple IO initialization, PCI device initialization, OS boot loader }
\end{center}

\end{figure}  

==> table.tex <==

{\small
\onecolumn
\begin{longtable}[c]{|c|cc|>{\scriptsize}c|c|c|c|c|c|c|c|}
\cline{4-11}
\multicolumn{2}{c}{}& & \multicolumn{8}{c|}{Role in System Trust } \\ 
\cline{4-11}
\multicolumn{2}{c}{}& & 
\multicolumn{2}{c}{Defensive model} &
\multicolumn{2}{c}{Attack} &
\multicolumn{2}{c}{Invisibility} &
\multicolumn{2}{c|}{Environment-awarity} 
\\ \cline{4-11}
\multicolumn{2}{c}{}& & 
\rotatebox{90}{ \small Modeling aspect\ }&
\rotatebox{90}{defense layer\ }&
\rotatebox{90}{attack\ }&
\rotatebox{90}{attacker layer\ }&
\rotatebox{90}{Technique\ }&
\rotatebox{90}{hidder layer\ }&
\rotatebox{90}{technique\ }&
\rotatebox{90}{Environmental aspect\ }
\\ \hline
\multirow{6}{*}{\begin{sideways}User level\end{sideways}} &   
\multicolumn{1}{|c}{\multirow{2}{*}{Application}} &
\multicolumn{1}{c|}{} & Transition model(CFI)\cite{CCFIR}& OS  &  &&&&&  \\
\multicolumn{1}{c|}{} & Selective Transition model(CPI)\cite{cpi}& OS  &  &&&&&  \\
\multicolumn{1}{|c|}{}        &                &  
\multicolumn{1}{c|}{} & Fault domain new abstraction (SFI)\cite{reins}\cite{sficisc} & Hypervisor  &  &&&&&  \\
\cline{2-11} &
\multicolumn{1}{|c}{\multirow{2}{*}{Interpreter}} &
\multicolumn{1}{c|}{} & 4 &  &  &&&    &&\\
\multicolumn{1}{|c|}{}        &                &  
\multicolumn{1}{c|}{}& 100.00\% &  &  &&&&&  \\
\cline{2-11} &
\multicolumn{1}{|c}{\multirow{2}{*}{OS serverces/libs}} &
\multicolumn{1}{c|}{} & 4 &  &  &&& &&\\
\multicolumn{1}{|c|}{}        &                &  
\multicolumn{1}{c|}{}& 100.00\% &  &  &&&&&\\
\hline
\multicolumn{2}{|c}{\multirow{2}{*}{Opertaing system}} &
\multicolumn{1}{c|}{} &  &  & 3 & 10&&&&    \\
\multicolumn{2}{|c}{}                 &  
\multicolumn{1}{c|}{}& 4 & 23 & 3 & 10&&&& \\
\hline
\multicolumn{2}{|c}{\multirow{2}{*}{VMM}} &
\multicolumn{1}{c|}{} & 4 & 23 & 3 & 10&&&&    \\
\multicolumn{2}{|c}{}                 &  
\multicolumn{1}{c|}{}& 4 & 23 & 3 & 10&&&& \\
\hline
\multicolumn{2}{|c}{\multirow{2}{*}{MLE}} &
\multicolumn{1}{c|}{} & 4 & 23 & 3 & 10&&&&    \\
\multicolumn{2}{|c}{}                 &  
\multicolumn{1}{c|}{}& 4 & 23 & 3 & 10&&&& \\
\hline

\multirow{6}{*}{\begin{sideways}Firmware\end{sideways}} &   
\multicolumn{1}{|c}{\multirow{2}{*}{SMM}} &
\multicolumn{1}{c|}{} & 4 &  &  &&&&&  \\
\multicolumn{1}{|c|}{}        &                &  
\multicolumn{1}{c|}{} & 100.00\% &  &  &&&&& \\
\cline{2-11} &
\multicolumn{1}{|c}{\multirow{2}{*}{SMT}} &
\multicolumn{1}{c|}{} & 4 &  &  &&&    &&\\
\multicolumn{1}{|c|}{}        &                &  
\multicolumn{1}{c|}{}& 100.00\% &  &  &&&&&  \\
\cline{2-11} &
\multicolumn{1}{|c}{\multirow{2}{*}{BIOS}} &
\multicolumn{1}{c|}{} & 4 &  &  &&&    &&\\
\multicolumn{1}{|c|}{}        &                &  
\multicolumn{1}{c|}{}& 100.00\% &  &  &&&&&  \\
\cline{2-11} &
\multicolumn{1}{|c}{\multirow{2}{*}{BIOS-verifier}} &
\multicolumn{1}{c|}{} & 4 &  &  &&& &&\\
\multicolumn{1}{|c|}{}        &                &  
\multicolumn{1}{c|}{}& 100.00\% &  &  &&&&&\\
\hline

\multicolumn{2}{|c}{\multirow{2}{*}{Out of band monitor}} &
\multicolumn{1}{c|}{} & 4 & 23 & 3 & 10&&&&    \\
\multicolumn{2}{|c}{}                 &  
\multicolumn{1}{c|}{}& 4 & 23 & 3 & 10&&&& \\
\hline
\multicolumn{2}{|c}{\multirow{2}{*}{TPM}} &
\multicolumn{1}{c|}{} & 4 & 23 & 3 & 10&&&&    \\
\multicolumn{2}{|c}{}                 &  
\multicolumn{1}{c|}{}& 4 & 23 & 3 & 10&&&& \\
\hline
\multicolumn{2}{|c}{\multirow{2}{*}{chipset}} &
\multicolumn{1}{c|}{} & 4 & 23 & 3 & 10&&&&    \\
\multicolumn{2}{|c}{}                 &  
\multicolumn{1}{c|}{}& 4 & 23 & 3 & 10&&&& \\
\hline
\multicolumn{2}{|c}{\multirow{2}{*}{CPU}} &
\multicolumn{1}{c|}{} & 4 & 23 & 3 & 10&&&&    \\
\multicolumn{2}{|c}{}                 &  
\multicolumn{1}{c|}{}& 4 & 23 & 3 & 10&&&& \\
\hline
\end{longtable} 
}
\twocolumn


==> table2.tex <==
\begingroup
\setlength{\tabcolsep}{7pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.1} % Default value: 1
{\scriptsize
\begin{center}
\begin{table}[ht]
    \begin{tabular}{ ? p{0.06cm} ? p{2.9cm} ? p{4.5cm} ?}
\specialrule{.2em}{.1em}{.1em}
    & Code execution unit & Summary \\ 
\specialrule{.2em}{.1em}{.1em}
    1& high-level executives  & codes require interpreters like Java, or run-time frameworks like .Net  \\ \hline    
    2& compiled executives  & ordinary applications.   \\ \hline
    3& application isolator & separated user-space environments like container, jail \\ \hline               	4& OS services/libraries  & User-space parts of operating system \\ \hline
    5& SW OS-virtualization & software virtual machines like Emulators, sandboxes \\ \hline
    6& Operating system kernel & main OS executive \\ \hline
    7& Drivers & Executives running in kernel space \\ \hline
    8& Hypervisor& Virtual machine monitors in HW virtualization scenario  \\ \hline  
    9& Measured Launch environment & like measured boot, late-launch sessions    \\ \hline  
    10& SMM code & SMI interrupt handler code   \\ \hline  
    11& option-ROM & The firmware for devices.  \\ \hline  
    12& UEFI & New firmware interface layer  \\ \hline
    13& BIOS & Firmware code for bootstrapping the system  \\ \hline  
    14& s-bridge devices & Devices connects to the south bridge  \\ \hline  %khode controller bus ham inja
    15& n-bridge devices & Devices connects to the north bridge  \\ \hline  
    16& out-of-band management &  Intel technology for remote monitoring of the system \\ \hline  
    17& chip-set (south/north bridges) &  Hardware chips for connecting devices to the CPU \\ \hline  
    18& Micro-codes & updatable codes to implement instructions  \\ \hline
    19& CPU hardwired code/state & CPU includes mainly hardwired codes as well as configuration registers  \\
    \specialrule{.2em}{.1em}{.1em}
    \end{tabular}
  \caption{Different code execution units found for a system with X86 architecture.}
  \label{execution-units}
\end{table}
\end{center}
}
\endgroup

==> table3.tex <==

{\scriptsize
\begin{table*}[h]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\cline{2-15}
\multicolumn{1}{c|}{} &\rotatebox{90}{user-level application} & \rotatebox{90}{user-level isolator} & \rotatebox{90}{SW virtual-machines} & \rotatebox{90}{OS libs/services}& \rotatebox{90}{OS}& \rotatebox{90}{Hypervisor} & \rotatebox{90}{MLE}& \rotatebox{90}{SMI code} & \rotatebox{90}{SMI monitor} & \rotatebox{90}{UEFI}& \rotatebox{90}{BIOS}& \rotatebox{90}{Co-processor}& \rotatebox{90}{Chipset}& \rotatebox{90}{microcodes}  \\
\hline
user-level applications & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
  & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
& \CheckmarkBold
 &  & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 \\
\hline
user-level isolation &  & \CheckmarkBold
 & \CheckmarkBold
  & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
& \CheckmarkBold
 &  & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 \\
\hline
SW virtual machines & &  & \CheckmarkBold
  & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
& \CheckmarkBold
 &  & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 \\
\hline
user-level OS libs/services  &  & &   & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
& \CheckmarkBold
 &  & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 \\
\hline
OS &  & &   &  & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
& \CheckmarkBold
 &  & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 \\
\hline
Hypervisor &  & &   & &  & \CheckmarkBold
 & \CheckmarkBold
& \CheckmarkBold
 &  & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 \\
\hline
MLE &  & &   & &  & & \CheckmarkBold
 & \CheckmarkBold
 & \checkmark
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 \\
\hline
SMI code &  & &   & &  &  &  & \CheckmarkBold
 & \checkmark
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 \\
\hline
SMI Monitor  &  & &   & &  &  &  &  & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 \\
\hline
UEFI &  & &   & &  &  &  &  {\color{red}\CheckmarkBold
} &  & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 \\
\hline
BIOS  &  & &   & &  &  &  & {\color{red}\CheckmarkBold
} &  &  & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 \\
\hline
Co-processors  &  & &   & &  &  &  &  &  &  & {\color{red}\CheckmarkBold
} & \CheckmarkBold
 & \CheckmarkBold
 & \CheckmarkBold
 \\
\hline
Chipset  &  & &   & &  &  &  &  &  &  &  &  & \CheckmarkBold
 & \CheckmarkBold
 \\
\hline
Microcodes &  & &   & &  &  &  &  &  &  & {\color{red}\CheckmarkBold
}& &  & \CheckmarkBold
 \\
\hline
\end{tabular}
\end{center}
\caption{Table caption.}
\label{INAM}
\end{table*}
}
